PASC-Net:Plug-and-play Shape Self-learning Convolutions Network with Hierarchical Topology Constraints for Vessel Segmentation

Accurate vessel segmentation is crucial to assist in clinical diagnosis by medical experts. However, the intricate tree-like tubular structure of blood vessels poses significant challenges for existing segmentation algorithms. Small vascular branches are often overlooked due to their low contrast compared to surrounding tissues, leading to incomplete vessel segmentation. Furthermore, the complex vascular topology prevents the model from accurately capturing and reconstructing vascular structure, resulting in incorrect topology, such as breakpoints at the bifurcation of the vascular tree. To overcome these challenges, we propose a novel vessel segmentation framework called PASC Net. It includes two key modules: a plug-and-play shape self-learning convolutional (SSL) module that optimizes convolution kernel design, and a hierarchical topological constraint (HTC) module that ensures vascular connectivity through topological constraints. Specifically, the SSL module enhances adaptability to vascular structures by optimizing conventional convolutions into learnable strip convolutions, which improves the network's ability to perceive fine-grained features of tubular anatomies. Furthermore, to better preserve the coherence and integrity of vascular topology, the HTC module incorporates hierarchical topological constraints-spanning linear, planar, and volumetric levels-which serve to regularize the network's representation of vascular continuity and structural consistency. We replaced the standard convolutional layers in U-Net, FCN, U-Mamba, and nnUNet with SSL convolutions, leading to consistent performance improvements across all architectures. Furthermore, when integrated into the nnUNet framework, our method outperformed other methods on multiple metrics, achieving state-of-the-art vascular segmentation performance.

==> com_table.tex <==

\begin{table*}[ht]
\caption{Quantitative comparison with the state-of-the-art methods on two public datasets}
\label{com}
\begin{center}
\renewcommand\arraystretch{1.4}
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hspace{30pt}}l@{\hspace{30pt}}l@{\hspace{30pt}}c@{\hspace{30pt}}c@{\hspace{30pt}}c@{\hspace{30pt}}c@{\hspace{30pt}}c@{\hspace{30pt}}c}
\toprule

Dataset  &Method      &Publication     & Dice(\%)$\uparrow$    &  IoU(\%)$\uparrow$  & Precision(\%)$\uparrow$ & Recall(\%)$\uparrow$ & clDice(\%)$\uparrow$& ASD$\downarrow$ \\  
\midrule
\multirow{9}{*}{Arcade}
&UNet\cite{ronneberger2015u}   & MICCAI 2015 & 72.61\scriptsize$\pm$0.74& 58.37\scriptsize$\pm$1.03& 73.06\scriptsize$\pm$1.05& 74.46\scriptsize$\pm$1.01&71.20\scriptsize$\pm$0.82& 11.88\scriptsize$\pm$0.78\\
\addlinespace[1ex]
&clDice\cite{shit2021cldice} &CVPR 2021 & 73.31\scriptsize$\pm$1.09& 59.73\scriptsize$\pm$1.31& 74.13\scriptsize$\pm$1.25& 77.31\scriptsize$\pm$1.47&75.81\scriptsize$\pm$1.16& 10.76\scriptsize$\pm$0.80\\
\addlinespace[1ex]
&ResUNet\cite{xiao2018weighted} &ITME 2018 & 73.39\scriptsize$\pm$0.81& 59.45\scriptsize$\pm$1.11& 76.15\scriptsize$\pm$0.95& 73.31\scriptsize$\pm$1.19&72.70\scriptsize$\pm$0.89& 11.20\scriptsize$\pm$0.62\\
\addlinespace[1ex]
&$\mathrm{CS}^{2}$-Net\cite{mou2021cs2} &MedIA 2021 & 76.99\scriptsize$\pm$0.53& 63.67\scriptsize$\pm$0.86& 77.69\scriptsize$\pm$0.90& 78.22\scriptsize$\pm$0.68&76.68\scriptsize$\pm$0.66& 9.82\scriptsize$\pm$0.47\\
\addlinespace[1ex]
&DSCNet\cite{qi2023dynamic}&ICCV 2023   & 77.48\scriptsize$\pm$0.55& 64.36\scriptsize$\pm$0.88& 78.79\scriptsize$\pm$0.95& 77.68\scriptsize$\pm$0.58&77.47\scriptsize$\pm$0.64& 9.36\scriptsize$\pm$0.52\\
\addlinespace[1ex]
&CoANet\cite{mei2021coanet} &TIP 2021  & 80.71\scriptsize$\pm$0.36& 68.47\scriptsize$\pm$0.65& 80.65\scriptsize$\pm$0.79& 82.53\scriptsize$\pm$0.43&81.79\scriptsize$\pm$0.52& 7.43\scriptsize$\pm$0.47\\
\addlinespace[1ex]
&U-Mamba\cite{ma2024u}       &arXiv 2024            & 80.00\scriptsize$\pm$0.56&67.84\scriptsize$\pm$0.89&80.01\scriptsize$\pm$0.79&81.61\scriptsize$\pm$0.77& 81.39\scriptsize$\pm$0.69&7.87\scriptsize$\pm$0.69\\
\addlinespace[1ex]
&nnUNet\cite{isensee2021nnu}   &Nat. Methods 2021      & 81.10\scriptsize$\pm$0.57& 69.42\scriptsize$\pm$0.93& 80.51\scriptsize$\pm$0.90& 83.24\scriptsize$\pm$0.62& 82.05\scriptsize$\pm$0.77& 7.52\scriptsize$\pm$0.62\\
\addlinespace[1ex]
&\textbf{Ours}           & ---------  & \textbf{82.39}\scriptsize$\pm$0.55& \textbf{71.21}\scriptsize$\pm$0.88& \textbf{82.76}\scriptsize$\pm$0.83& \textbf{83.54}\scriptsize$\pm$0.69& \textbf{83.50}\scriptsize$\pm$0.72& \textbf{6.77}\scriptsize$\pm$0.54\\
\midrule
\multirow{9}{*}{FIVES}
&UNet\cite{ronneberger2015u}   & MICCAI 2015          & 80.80\scriptsize$\pm$1.34& 70.26\scriptsize$\pm$1.68& \textbf{94.35}\scriptsize$\pm$0.17& 73.56\scriptsize$\pm$1.92&81.77\scriptsize$\pm$1.29& 11.75\scriptsize$\pm$5.72\\
\addlinespace[1ex]
&clDice\cite{shit2021cldice}   &CVPR 2021          & 85.92\scriptsize$\pm$0.76& 76.84\scriptsize$\pm$1.04& 92.44\scriptsize$\pm$0.28& 81.71\scriptsize$\pm$1.15&87.30\scriptsize$\pm$0.75& 8.29\scriptsize$\pm$3.06\\
\addlinespace[1ex]
&ResUNet\cite{xiao2018weighted}  &ITME 2018        & 84.62\scriptsize$\pm$0.92& 75.15\scriptsize$\pm$1.24& 93.40\scriptsize$\pm$0.25& 79.41\scriptsize$\pm$1.43&86.91\scriptsize$\pm$0.88& 8.37\scriptsize$\pm$2.86\\
\addlinespace[1ex]
&$\mathrm{CS}^{2}$-Net\cite{mou2021cs2} &MedIA 2021 & 88.59\scriptsize$\pm$0.55         & 80.71\scriptsize$\pm$0.84        & 93.90\scriptsize$\pm$0.21& 84.49\scriptsize$\pm$0.79&88.62\scriptsize$\pm$0.54& 5.90\scriptsize$\pm$0.71\\
\addlinespace[1ex]
&DSCNet\cite{qi2023dynamic}    &ICCV 2023          & 88.57\scriptsize$\pm$0.53         & 80.61\scriptsize$\pm$0.79        & 92.53\scriptsize$\pm$0.22& 85.53\scriptsize$\pm$0.72&88.70\scriptsize$\pm$0.53& 6.43\scriptsize$\pm$1.20\\
\addlinespace[1ex]
&CoANet\cite{mei2021coanet}   &TIP 2021             & 89.66\scriptsize$\pm$0.50         & 82.30\scriptsize$\pm$0.71        & 94.11\scriptsize$\pm$0.12& 86.27\scriptsize$\pm$0.67&89.76\scriptsize$\pm$0.49& 5.47\scriptsize$\pm$0.87\\
\addlinespace[1ex]
&U-Mamba\cite{ma2024u}         &arXiv 2024           & 89.39\scriptsize$\pm$0.50         & 81.86\scriptsize$\pm$0.71        & 90.18\scriptsize$\pm$0.18& 89.28\scriptsize$\pm$0.67&89.67\scriptsize$\pm$0.52& 6.25\scriptsize$\pm$0.81\\
\addlinespace[1ex]
&nnUNet\cite{isensee2021nnu}    &Nat. Methods 2021         & 89.40\scriptsize$\pm$0.49         & 81.87\scriptsize$\pm$0.71        & 91.09\scriptsize$\pm$0.21& 88.30\scriptsize$\pm$0.68&89.20\scriptsize$\pm$0.53& 7.47\scriptsize$\pm$1.33\\
\addlinespace[1ex]
&\textbf{Ours}                &  ---------         & \textbf{91.83}\scriptsize$\pm$0.43&\textbf{85.83}\scriptsize$\pm$0.63& 93.44\scriptsize$\pm$0.12& \textbf{90.97}\scriptsize$\pm$0.55&\textbf{91.74}\scriptsize$\pm$0.42& \textbf{4.69}\scriptsize$\pm$0.66\\

\bottomrule
\end{tabular}}
\end{center}
\end{table*}
